Data-based optimal estimation of frequency bias: The case of Southwest Power Pool

In this paper, we introduce a method to optimally estimate time-varying frequency bias. Current industry practice is to assume that frequency bias is changing only on annual basis. We suggest that this improved time-dependent bias estimate can be used to reduce the cost of frequency regulation needed to meet industry standards requested by the North American Electric Reliability Corporation (NERC). Optimization of time-varying frequency bias is posed as a parameter estimation (calibration) problem whose implementation utilizes online system measurements. It is further shown how this result can be used to estimate intra-dispatch load deviations. This knowledge is needed to estimate more accurately regulation reserve needed, and to therefore reduce overall regulation cost. Methods can be introduced to give incentives to demand response to participate in frequency regulation. Overall, we show the importance of incorporating knowledge of physics-based models for data-enabled parameter estimation of physical systems.

==> text/NAI.tex <==
\section{Discussion on poorly estimated frequency bias effects} %{Data enabled NAI estimation}

Inadvertent energy exchange (IEE) is created
by the difference of hourly NAI and Net Scheduled Interchange (NSI). This effect is produced because generation
cannot physically follow the demand of the system, and that is why supplemental control is used. In other words, when the IEE within an CA no longer sums to zero, there
will exist a generation surplus which will show up in the frequency deviations. IEE should be equal to zero if the $NAI[kTs]$ is equal to the $NSI[kTs]$ for that hour. The goal of each CA is to appropriately manage its
IEE accumulations. 

As can be seen with the constant value of the frequency bias NAI and NSI are

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{img/nsi.png}
\caption{\label{fig:nasi}  NAI and NSI for 11-04-2017 on a minut basis }
\end{figure}

And if there is an optimal value of frequency bias then through the equations ~\ref{eq:aceinter} and ~\ref{eq:acesum} and ~\ref{eq:acef} we can see that IEE on hourly basis would be 

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{img/oatielf.png}
\caption{\label{fig:nasi}  IEE and optimal IEE for 11-04-2017 on a minut basis}
\end{figure}

It can be seen that on the average optimal IEE is greater than IEE obtained for the fixed frequency bias.
